Urban Sound Propagation: a Benchmark for 1-Step Generative Modeling of Complex Physical Systems

Data-driven modeling of complex physical systems is receiving a growing amount of attention in the simulation and machine learning communities. Since most physical simulations are based on compute-intensive, iterative implementations of differential equation systems, a (partial) replacement with learned, 1-step inference models has the potential for significant speedups in a wide range of application areas. In this context, we present a novel benchmark for the evaluation of 1-step generative learning models in terms of speed and physical correctness. Our Urban Sound Propagation benchmark is based on the physically complex and practically relevant, yet intuitively easy to grasp task of modeling the 2d propagation of waves from a sound source in an urban environment. We provide a dataset with 100k samples, where each sample consists of pairs of real 2d building maps drawn from OpenStreetmap, a parameterized sound source, and a simulated ground truth sound propagation for the given scene. The dataset provides four different simulation tasks with increasing complexity regarding reflection, diffraction and source variance. A first baseline evaluation of common generative U-Net, GAN and Diffusion models shows, that while these models are very well capable of modeling sound propagations in simple cases, the approximation of sub-systems represented by higher order equations systematically fails. Information about the dataset, download instructions and source codes are provided on our website: https://www.urban-sound-data.org.

==> sections/X_datasheet_for_dataset.tex <==

\section{Datasheets for Datasets}
\label{sec:appendix_datasheets_for_datasets}

\subsection{Motivation}

\textbf{For what purpose was the dataset created?} Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description.\\
{\fontfamily{cmr}\selectfont
Generative models, through their capacity to learn from complex datasets, hold significant potential in understanding the intricate physics behind sound propagation. By training on data that encompasses various urban layouts and the corresponding sound distribution maps, these models can uncover the underlying patterns and principles governing how sound travels and interacts with different obstacles, such as buildings and open spaces. This capability enables the creation of predictive models that can simulate sound behavior in any urban environment, thereby offering valuable insights for urban planning, acoustic design, and noise mitigation strategies, all rooted in a deep understanding of the physical laws of sound propagation.
}
\\
\\
\textbf{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}\\
{\fontfamily{cmr}\selectfont
Anonymous for Blind Review
}
\\
\\
\textbf{Who funded the creation of the dataset?} If there is an associated grant, please provide the name of the grantor and the grant name and number.\\
{\fontfamily{cmr}\selectfont
Anonymous for Blind Review
}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Composition}

\textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?} Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between them; nodes and edges)? Please provide a description.\\
{\fontfamily{cmr}\selectfont
A data point in this dataset consists of two main components: an urban layout image from OpenStreetMap and a corresponding sound distribution map. The urban layout image is a 500m x 500m area depiction where buildings are marked in black and open spaces in white. The sound distribution map, generated using NoiseModelling v4.0, illustrates the sound dynamics within that urban environment at resolutions of 512x512 or 256x256.
}



\textbf{How many instances are there in total (of each type, if appropriate)?}\\
{\fontfamily{cmr}\selectfont
The dataset is segmented into four distinct subsets, each tailored to explore specific aspects of sound propagation in urban environments: Baseline, Reflection, Diffraction, and Combined. Number of Instances: ~100,000.
}
\\
\\
\textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?} If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).\\
{\fontfamily{cmr}\selectfont
The dataset contains all generated instances.
}
\\
\\
\textbf{What data does each instance consist of?} “Raw” data (e.g., unprocessed text or images) or features? In either case, please provide a description.\\
{\fontfamily{cmr}\selectfont
A data point in this dataset includes an urban layout image from OpenStreetMap, showing a 500m x 500m area with buildings in black and open spaces in white, alongside a sound distribution map at 512x512 or 256x256 resolutions, created with NoiseModelling v4.0 to depict sound dynamics. Additionally, it incorporates environmental factors such as humidity, source decibels, and temperature, enriching the context for sound propagation analysis.
}
\\
\\
\textbf{Is there a label or target associated with each instance?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
Yes, each instance in our dataset is associated with a label or target. This information is organized within a CSV file, which includes mappings between the OSM images and their corresponding simulation outputs. Additionally, the CSV file contains descriptive variables for each sample. To facilitate easy identification and correlation, the sample ID is also embedded in the filename of each image. 
}
\\
\\
\textbf{Is any information missing from individual instances?} If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g., redacted text.\\
{\fontfamily{cmr}\selectfont
No information is missing. 
}
\\
\\
\textbf{Are relationships between individual instances made explicit (e.g., users’ movie ratings, social network links)?} If so, please describe how these relationships are made explicit.\\
{\fontfamily{cmr}\selectfont
No, there are no explicit relationships between individual instances in our dataset. Each instance stands independently and is not linked to others.
}
\\
\\
\textbf{Are there recommended data splits (e.g., training, development/validation, testing)?} If so, please provide a description of these splits, explaining the rationale behind them.\\
{\fontfamily{cmr}\selectfont
For our study, we have adopted a data split of 80/15/5, which means 80\% of the data is used for training, 15\% for development or validation, and the remaining 5\% for testing.
}
\\
\\
\textbf{Are there any errors, sources of noise, or redundancies in the
dataset?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
None.
}
\\
\\
\textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)?} If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a dataset consumer? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.\\
{\fontfamily{cmr}\selectfont
The dataset is self-contained and does not link to external resources.
}
\\
\\
\textbf{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor–patient confidentiality, data that includes the content of individuals’ non-public communications)?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
No, there are no personal data included in the dataset.
}
\\
\\
\textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}
If so, please describe why.\\
{\fontfamily{cmr}\selectfont
No, such data does not exist in the dataset.
}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Collection Process}

\textbf{How was the data associated with each instance acquired?} 
Was the data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If the data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.\\

{\fontfamily{cmr}\selectfont
The data for each instance in our dataset was acquired directly using the Overpass API, which provides OpenStreetMap data. This process involves retrieving raw data, and we did not undertake any further verification or validation steps.
}
\\
\\
\textbf{What mechanisms or procedures were used to collect the data
(e.g., hardware apparatuses or sensors, manual human curation,
software programs, software APIs)?} How were these mechanisms or
procedures validated?\\
{\fontfamily{cmr}\selectfont
The following procedures were used to collect the data:
\begin{enumerate}
    \item 
\end{enumerate}

}
\textbf{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling probabilities)?}\\
{\fontfamily{cmr}\selectfont
The dataset is not a sample from a larger set.
}
\\
\textbf{Who was involved in the data collection process (e.g., students,
crowdworkers, contractors) and howwere they compensated (e.g.,
how much were crowdworkers paid)?}\\
{\fontfamily{cmr}\selectfont
 Anonymous for Blind Review
}
\textbf{Over what timeframe was the data collected?} 
Does this timeframe
match the creation timeframe of the data associated with the instances
(e.g., recent crawl of old news articles)? If not, please describe the timeframe in which the data associated with the instances was created.\\
{\fontfamily{cmr}\selectfont
10/2023 - 12/2023
}
\textbf{Were any ethical review processes conducted (e.g., by an institutional review board)?} If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.\\
{\fontfamily{cmr}\selectfont
There is no personal data collection from the people who are created the dataset.
}
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Preprocessing/cleaning/labeling}

\textbf{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?} If so, please provide a description. If not, you may skip the
remaining questions in this section.\\
{\fontfamily{cmr}\selectfont
There are some entities that group arbitrary products due to manual miss-annotations of the GTINs to these products.
Because of this occurrence, cake baking mix, cream, and pudding form an entity.
We eliminated many images that have been labeled wrongly to clean the dataset.
However, there is no guarantee that we did not miss more and less obvious of these cases.
}
\\
\\
\textbf{Was the “raw” data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?} If so, please provide a link or other access point to the “raw” data.\\
{\fontfamily{cmr}\selectfont
No, the "raw" data is not saved separately. 
The leaflets being the basis for the dataset creation are stored at the company internally.
}
\\
\\
\textbf{Is the software that was used to preprocess/clean/label the data available?} If so, please provide a link or other access point.\\
{\fontfamily{cmr}\selectfont
No, the cleaning of the data was done by manual screening. There is no code / software available.
}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Uses}

\textbf{Has the dataset been used for any tasks already?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
The dataset itself has not been used for any tasks already. 
But a subset of the dataset was used company internally for the price monitoring service.
}
\\
\\
\textbf{Is there a repository that links to any or all papers or systems that use the dataset?} If so, please provide a link or other access point.\\
{\fontfamily{cmr}\selectfont
No, there is no repository.
}
\\
\\
\textbf{What (other) tasks could the dataset be used for?}\\
{\fontfamily{cmr}\selectfont
The dataset can be also used for the image classification or the image retrieval task. Both tasks are investigated in our experiments. Unfortunately, they do not solve the visual EM problem. Furthermore, the images in the dataset can be used for the OCR task. But the Ground Truth data of the text in the images is not provided by our dataset.
}
\\
\\
\textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?} For example, is there anything that a dataset consumer might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other risks or harms (e.g., legal risks, financial harms)? If so, please provide a description. Is there anything a dataset consumer could do to mitigate these risks or harms?\\
{\fontfamily{cmr}\selectfont
Unknown to the authors of the datasheet.
}
\\
\\
\textbf{Are there tasks for which the dataset should not be used?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
Unknown to the authors of the datasheet.
But the license of the dataset prohibits commercial purpose and the distribution of a modified version of the dataset.}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Distribution}

\textbf{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?} If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
Yes, the dataset is publicly available on the internet.
}
\\
\\
\textbf{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?} Does the dataset have a digital object identifier (DOI)?\\
{\fontfamily{cmr}\selectfont
Information about the dataset and code as well as the downloading steps will be provided after acceptance.
The dataset can be also downloaded directly via the URL \url{https://zenodo.org/record/797056}. 
The DOI of the dataset is 10.5281/zenodo.7970566.
}
\\
\\
\textbf{When will the dataset be distributed?}\\
{\fontfamily{cmr}\selectfont
The dataset was released at Jun 06, 2023.
}
\\
\\
\textbf{Will the dataset be distributed under a copyright or other intellectual
property (IP) license, and/or under applicable terms of use (ToU)?} If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.\\
{\fontfamily{cmr}\selectfont
This dataset is licensed under the \textit{Creative Commons Attribution-NonCommercial-NoDerivatives 4.0 International} license. For more information about the license see \url{https://creativecommons.org/licenses/by-nc-nd/4.0/}.
}
\\
\\
\textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?} If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.\\
{\fontfamily{cmr}\selectfont
Unknown to the authors of the datasheet.
}
\\
\\
\textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.\\
{\fontfamily{cmr}\selectfont
Unknown to the authors of the datasheet.
}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}

\subsection{Maintenance}
\label{subsec:maintenance}

\textbf{Who will be supporting/hosting/maintaining the dataset?}\\
{\fontfamily{cmr}\selectfont
The research group of the institution is supporting/maintaining the dataset.
}
\\
\\
\textbf{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}\\
{\fontfamily{cmr}\selectfont
The curators of the dataset can be contacted via info@Retail-786k.org.
}
\\
\\
\textbf{Is there an erratum?} If so, please provide a link or other access point.\\
{\fontfamily{cmr}\selectfont
No.
}
\\
\\
\textbf{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?} If so, please describe how often, by whom, and how updates will be communicated to dataset consumers (e.g., mailing list, GitHub)?\\
{\fontfamily{cmr}\selectfont
In the future, another version of the dataset could be published with information about price, discount, brand, and so on of the products per instance.\\
There is no fixed date for the upload of the new version, yet. Also, there will be no fixed periods for updating the dataset.\\
The new versions will be updated by the authors of the datasheet.
}
\\
\\
\textbf{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were the individuals in question told that their data would be retained for a fixed period of time and then deleted)?} If so, please describe these limits and explain how they will be enforced.\\
{\fontfamily{cmr}\selectfont
The dataset does not relate to people.
}
\\
\\
\textbf{Will older versions of the dataset continue to be supported/hosted/maintained?} If so, please describe how. If not, please describe how its obsolescence will be communicated to dataset consumers.\\
{\fontfamily{cmr}\selectfont
There are no older versions of the dataset, yet.
If newer versions are available, then old version will still be available.
}
\\
\\
\textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?} If so, please provide a description. Will these contributions be validated/verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to dataset consumers? If so, please provide a description.\\
{\fontfamily{cmr}\selectfont
The license of our dataset does not allow to extend/augment/build on/contribute to the dataset. Interested persons can contact the curators via info@Retail-786k.org.
}
\\
\\
\textbf{Any other comments?}\\
{\fontfamily{cmr}\selectfont
None.
}
